Predicting Long-Term Student Outcomes from Short-Term EdTech Log Data

Educational stakeholders are often particularly interested in sparse, delayed student outcomes, like end-of-year statewide exams. The rare occurrence of such assessments makes it harder to identify students likely to fail such assessments, as well as making it slow for researchers and educators to be able to assess the effectiveness of particular educational tools. Prior work has primarily focused on using logs from students full usage (e.g. year-long) of an educational product to predict outcomes, or considered predictive accuracy using a few minutes to predict outcomes after a short (e.g. 1 hour) session. In contrast, we investigate machine learning predictors using students' logs during their first few hours of usage can provide useful predictive insight into those students' end-of-school year external assessment. We do this on three diverse datasets: from students in Uganda using a literacy game product, and from students in the US using two mathematics intelligent tutoring systems. We consider various measures of the accuracy of the resulting predictors, including its ability to identify students at different parts along the assessment performance distribution. Our findings suggest that short-term log usage data, from 2-5 hours, can be used to provide valuable signal about students' long-term external performance.

==> sections/intro.tex <==
\section{Introduction}
%% short-long term prediction on CBLP
% understanding in terms of population and interventions, hard to measure external tests and re-run the system

% what is the problem
% why is it important and hard
%.  student identification. might be useful for interventions later (requires causality)
% key limitations of prior work
%.   most on full long data
%.   limited on data, very short. 
%.   shortening assessment (different, not expecting learning during this)
% insight
%.    may be feasible
%.    explore how good this is
% what can we do now
%    show across 3 domains. 

Though educational software, including intelligent tutors and educational games, is increasingly ubiquitous, evaluating the effectiveness of such software remains a challenge, at both an individual level and a population level. Typically school districts are most interested in long term student outcomes, like end of year state or national assessments. Though such assessments are often highly rigorous and carefully designed, their rare occurrence introduces multiple challenges, making it harder to identify students likely to fail such assessments, and making it slow 
for researchers, educators, product designers and policy makers to be able to assess the effectiveness of particular educational tools. It has long been recognized (see the Assistments literature (XX add citations)) that the logs generated when students interact with educational software could themselves be used as a form of temporally integrated insight into a student's state of knowledge. In this work we investigate machine learning predictors using students' logs during their first few hours of use with educational technology can provide useful predictive insight into those students' end-of-school year external assessment. 

There are multiple reasons such predictors would be helpful. Such predictors might be used within the software itself, to help introduce different forms of pedagogical instruction and support to students who are struggling, or even new challenges to those that are thriving. While many educational tools already involve some aspects of personalization, to our knowledge such tools typically rely on basing such personalization given other proxy measures of student outcomes (such as performance on a set of internally defined skills). While there is some prior work relating such proxies as observed over the school year to external assessments (**cite Fancsali and APLSE), it is unclear if such features as observed over a full year are necessarily predictive given only a limited window, which is important if these shorter term signals are used for instructional decisions. In general, it is unclear if many software educational products are carefully aligning short term outcomes used to make automated instructional decisions, towards maximizing desired long term outcomes: indeed, doing so has often been very challenging due to the time horizons involved. 

Equally importantly, this information could be provided to teachers to help them better understand the progress of individual students and their class as a whole, potentially informing the need for additional resources or changes in strategy. For example, a teacher might assign an aide to spend more time with a struggling student, or a fifth grade teacher might choose to increase the amount of time spent on math if their whole class is expected to perform poorly. 

% evaluate new instruction (but do this later)

Though such tools would be very useful, it is unclear apriori if very limited, on the order of 1-3 hours, data from students' interactions with an educational tutor, can be used to predict assessments taken months later. Indeed, to our knowledge there has been very limited prior work on using such short horizon log data to predict delayed long term outcomes. 

Rather, prior work has tackled other related aspects to the problem we consider. First, there have been a number of papers showing that using long horizon student data logs can be used to help predict external assessments, across multiple intelligent tutoring systems and educational software products, including Cognitive Tutor (**cite both papers from Fancsali), Assistments (**cite Heffernan's work) (**add others). Such work has typically shown that log data provides a useful signal to help predict student tests scores, focusing on population measures like Pearson correlation and root mean squared error. Recently, perhaps in part motivated by the significant challenges during the covid-19 pandemic of conducting standard educational assessments when many students are remote, people have been interested in designing much shorter assessments that have similar benefits to existing, much longer assessments-- for example, (**cite yateman) developed a reading assessment that can be done in 2 minutes that has YYY and ZZZ. In such settings the assumption is that the assessment is being done to capture static student performance, rather than extracting signal  during standard usage of a product designed to support student learning.\footnote{An interesting possibility if very short test become feasible is whether they could be more widely incorporated in standard software, so as not to distract from learning, which is often a challenge with lengthy assessments.}

Most related to our current work is a couple recent papers that have similarly examined whether very short term data from student log outcomes can predict more delayed student outcomes (**cite both papers). However, in both settings the length of duration was very short, focused on a single session of interaction with a student: 
in one case, the authors examined how performance on the first problem related to post test after 12 problems, and in another they looked at performance on the first XX minutes related to the final outcome after 20 minutes. While such work has a related motivation, in contrast, in our work we are interested in much longer time scales, seeking to use a limited amount of likely multi-session data to predict external assessments taken months later to evaluate student learning (and the impact of educational support) on much broader scale. In addition, to our knowledge this prior work, and the research that has developed predictors of external student assessments using many session (e.g. school year) student tutoring logs, has analyzed performance on a single educational tool and/or  platform, leaving open trends and similarities across educational technology systems.

We note that there has been significant work on developing surrogate measures of delayed outcomes in social science and economics: here such surrogates are expected to satisfy a causal relationship, such that when observed, the surrogate measure renders the down stream outcome independent of the prior intervention, such as predicting employment many years after a short term job training program, using a surrogate of 1 year employment status~\cite{athey2019surrogate}. Surrogate endpoints are also used in clinical settings, when the desired outcome of interest may be substantially delayed (such as 5 year survival rates) and when other shorter term measures are known to be predictive of the long term outcome.\footnote{https://www.fda.gov/about-fda/innovation-fda/fda-facts-biomarkers-and-surrogate-endpoints}, and increasingly in other settings 
%measured~\citep{hohnhold2015focusing,ritter2013predicting}. 
such as finance and recommendation systems~\citep{wang2022surrogate,zhang2023evaluating,hohnhold2015focusing}.  



Another challenging situation is that available observations of students can be commonly limited. Prior works have found some powerful indicators (e.g., demographics, pre-test scores, knowledge components (KCs)) to predict students' outcomes at an early stage~\citep{acharya2014early,ritter2013predicting,zheng2019using,alhazmi2023early}. However, those information may not always be available to tutors. And most of the prior works mainly focused on a specific platform or context, there is lack investigation on what features might be generally important across contexts to guide tutors from a new context to quickly understand the potential future outcomes of students. 

Third, while a crucial goal for developing new tools and interventions is broadly enhancing learning outcomes over student populations, it is also pivotal to understand its potential effects on varied students subgroups sorted by performance at an early stage, since we would like to understand whether various performers could benefit from new interventions. However, prior work mainly focus on developing techniques to enhance prediction on specific subgroups (\textit{e.g.},~\citep{helal2019identifying}), while we are particularly interested in evaluating over both population and subgroups during predicting long-term outcomes, with respect to short horizon and the sets of predictive features.      

% who struggle at an early stage without timely support can result in undesirable outcomes, such as failing the course. However, identifying students in-need within a short period can be hard, given their underlying mindsets are generally unknown, and their information (e.g., demographics, grades of prior courses, etc.) could be limited. 



%% RQs
In this work, we investigate the prediction of long-term, external students' outcomes using their short-horizon log data, across tutoring systems across three different educational contexts: the Can't Wait to Learn reading educational technology games (using data from students in Uganda), iReady middle school math intelligent tutor (used by seventh graders in the United States) and Mathia middle school math intelligent tutor (used by XXX graders in the United states).  We explore the potential of using short horizon features that could be generally extracted from log data across contexts, without extensive domain knowledge of the underlying educational software tool or student demographics or student prior performance data. We do this in part such student data may not always be available for many reasons, including the common case of new students who transfer to a new district, particularly midway through an academic year. In addition, by focusing on broadly similar features that are likely to be present across many educational platforms, we can evaluate the similarities and differences across settings. Using such features, we compare the performance of three popular machine learning models (\textit{i.e.}, linear regression, support vector regression, and random forest) with respect to the length of horizon and contexts. 

While prior work has primarily focused on population level metrics, part of the motivation for such work is the potential to help support students who are expected to have major challenges months later on an external assessment if their trajectory continues, or to potentially celebrate or challenge a student that is already showing signs of strong expected future performance. To investigate this further, we also analyze the resulting quality of the short-horizon estimates over subgroups of students that are sorted by performance for a more thorough understanding about the prediction performance. Moreover, we examine the effects of pre-assessments on predictions over both population and subgroups, with different set of features, to understand if pretest data, when available, is similar, different or complimentary, to student log data. 
Specifically, we explore the following research questions:
\begin{enumerate}
    \item Can we consistently, across multiple educational tools, obtain a short-horizon log data only predictor of student long-term outcomes which provides significant predictive power on external, much delayed educational assessment? How does its accuracy compare to using the full log horizon data, and does performance versus horizon  vary by datasets/settings?
    \item Does the machine learning algorithms used to form the predictors significantly impact the resulting accuracy of the external assessment predictor?
    \item Is there a stable set of log data features across domains and datasets that is needed to form accurate short-horizon predictors of long-term outcomes? Are multiple features important for improving accuracy? %(all still with no pretest)? 
    \item What is the resulting quality of the short-horizon estimates and how does it differ across subgroups of students sorted by performance? % (are there other features of students that are relevant?)
    Are we systematically better or worse at predicting higher/lower performers?
    \item When pre-assessments are available, is the quality of using log data equivalent to this form of information, and do we see additive gains of combining both? 
\end{enumerate}



==> sections/older_intro.tex <==
\section{Introduction}
%% short-long term prediction on CBLP
% understanding in terms of population and interventions, hard to measure external tests and re-run the system
Advanced educational technologies (\textit{e.g.}, intelligent tutors, games, etc.) have been extensively employed world-widely to enhance student learning with appropriate activities and interventions. Developing and delivering new tools or interventions to students can be highly time- and resource consuming, especially when targeting their long-term outcomes with external measure, such as a global standardized test. A common way for determining whether a new intervention should be deployed is using short-term A/B tests. However, it can be less matching to the true outcome in long-term external measurements, while the long-term outcomes are not easy to be directly or frequently measured~\citep{hohnhold2015focusing,ritter2013predicting}. Predicting long-term outcomes using short-horizon data can be a potential way to decide an intervention to be deployed to students in a safer, more effective and efficient manner, which has raised attention and achieved desirable outcomes in various domains such as finance and recommendation systems~\citep{wang2022surrogate,zhang2023evaluating,hohnhold2015focusing}.  

In education, prior works have broadly investigated early prediction of students outcomes by using types of information, such as demographics, grades of prior course, click-stream data, etc. Many of the related work mainly focus on using a fixed, pre-defined short horizon, such as first several minutes after beginning of interaction and the first assignment, to predict students performance in a given course or test (\textit{e.g.},~\citep{mao2019one,gao2021early,}). while it's not clear how to select the length of horizon and whether that would effect prediction performance in a different educational context. And the target long-term outcome measure can be much longer and more high-stake, \textit{e.g.}, a national test one year after the beginning of interaction, compared to course grades within a semester or session, which requires more thorough investigation for stable predictors.  

Another challenging situation is that available observations of students can be commonly limited. Prior works have found some powerful indicators (e.g., demographics, pre-test scores, knowledge components (KCs)) to predict students' outcomes at an early stage~\citep{acharya2014early,ritter2013predicting,zheng2019using,alhazmi2023early}. However, those information may not always be available to tutors. And most of the prior works mainly focused on a specific platform or context, there is lack investigation on what features might be generally important across contexts to guide tutors from a new context to quickly understand the potential future outcomes of students. 

Third, while a crucial goal for developing new tools and interventions is broadly enhancing learning outcomes over student populations, it is also pivotal to understand its potential effects on varied students subgroups sorted by performance at an early stage, since we would like to understand whether various performers could benefit from new interventions. However, prior work mainly focus on developing techniques to enhance prediction on specific subgroups (\textit{e.g.},~\citep{helal2019identifying}), while we are particularly interested in evaluating over both population and subgroups during predicting long-term outcomes, with respect to short horizon and the sets of predictive features.      

% who struggle at an early stage without timely support can result in undesirable outcomes, such as failing the course. However, identifying students in-need within a short period can be hard, given their underlying mindsets are generally unknown, and their information (e.g., demographics, grades of prior courses, etc.) could be limited. 



%% RQs
In this work, we investigate the prediction of long-term, external students' outcomes using their short-horizon log data, across tutoring systems across three different educational contexts. We explore the effects of selecting length of short horizon on long-term outcomes of students with a set of features that could be generally extracted from log data across contexts. Also, we compare the performance of three popular machine learning models (\textit{i.e.}, linear regression, support vector regression, and random forest) with respect to the length of horizon and contexts. We further investigate the resulting quality of the short-horizon estimates over subgroups of students that are sorted by performance for a more thorough understanding about the prediction performance. Moreover, we examine the effects of pre-assessments on predictions over both population and subgroups, with different set of features. 
Specifically, we explore the following research questions:
\begin{enumerate}
    \item Can we consistently, across multiple domains and settings, obtain a short-horizon log data only predictor of student long-term outcomes that is as accurate as using the full horizon data? If so, does the length of the horizon needed vary by datasets/settings?
    \item Does the machine learning algorithms used to form the predictors significantly impact the resulting accuracy?
    \item Is there a stable set of log data features across domains and datasets that is needed to form accurate short-horizon predictors of long-term outcomes? Are multiple features important for improving accuracy? %(all still with no pretest)? 
    \item What is the resulting quality of the short-horizon estimates and how does it differ across subgroups of students sorted by performance? % (are there other features of students that are relevant?)
    Are we systematically better or worse at predicting higher/lower performers?
    \item When pre-assessments are available, is the quality of using log data equivalent to this form of information, and do we see additive gains of combining both? 
\end{enumerate}


